Integrated Gradient attribution for Gaussian Processes with non-Gaussian likelihoods

Gaussian Process (GP) models are a powerful tool in probabilistic machine learning with a solid theoretical foundation. Thanks to current advances, modeling complex data with GPs is becoming increasingly feasible, which makes them an interesting alternative to deep learning and related approaches. As the latter are getting more and more influential on society, the need for making a model's decision making process transparent and explainable is now a major focus of research. A major direction in interpretable machine learning is the use of gradient-based approaches, such as Integrated Gradients, to quantify feature attribution, locally for a given datapoint of interest. Since GPs and the behavior of their partial derivatives are well studied and straightforward to derive, studying gradient-based explainability for GPs is a promising direction of research. Unfortunately, partial derivatives for GPs become less trivial to handle when dealing with non-Gaussian target data as in classification or more sophisticated regression problems. This paper therefore proposes an approach for applying Integrated Gradient-based explainability to non-Gaussian GP models, offering both analytical and approximate solutions. This extends gradient-based explainability to probabilistic models with complex likelihoods to extend their practical applicability.

==> featatt/classification.tex <==
As $\tilde{f}$ and $\tilde{f}^{\partial_k}$ are correlated Gaussians as well, we can reduce the binary classification case in \eqref{meanbinary} to depend only on a single random variable:

\begin{corollary}
    \begin{equation}\label{expsimple}
        \begin{gathered}
            \mathbb{E}\left[\sigma'(\tilde{f})\cdot \tilde{f}^{\partial_k}\right] 
            = \mathbb{E}\left[\sigma'(\tilde{f}) \left(\tilde{m}^{\partial_k}+\frac{\tilde{k}^{\partial_k}}{\tilde{k}}(\tilde{f}-\tilde{m})\right)\right]
        \end{gathered}
    \end{equation}
\end{corollary}

Similarly, we get for the $C$-ary case:

\begin{corollary}
\begin{equation}\label{carymean}
    \begin{gathered}
        \mathbb{E}\Bigg[S(\tilde{f}_1,...,\tilde{f}_C)_{(c)}\cdot \tilde{f}_c^{\partial_k}\\
        -S(\tilde{f}_1,...,\tilde{f}_C)_{(c)}\cdot \frac{\sum_{j=1}^C exp(\tilde{f}_j)\cdot \tilde{f}_j^{\partial_k}}{\sum_{j=1}^C exp(\tilde{f}_j)}\Bigg]\\
        = \mathbb{E}\left[\tilde{S}_{(c)} \cdot \left\{m_c^{\partial_k}+\Sigma_{\tilde{f}\tilde{f}_c^{\partial_k}}\Sigma^{-1}_{\tilde{f}} \left(\tilde{f}-m_{\tilde{f}}\right)\right\}\right]\\
        -\sum_{j=1}^C \mathbb{E}\left[\tilde{S}_{(jc)}\cdot\left\{m_{j}^{\partial_k}+\Sigma_{\tilde{f}\tilde{f}_j^{\partial_k}}\Sigma^{-1}_{\tilde{f}}\left(\tilde{f}-m_{\tilde{f}}\right)\right\}\right]\\
    \end{gathered}
\end{equation}

\noindent where $\tilde{f}=\left[\tilde{f}_1,...,\tilde{f}_C\right]^T$, $m_{\tilde{f}}=\left[\mathbb{E}[\tilde{f}_1],...,\mathbb{E}[\tilde{f}_C]\right]^T$,  $\tilde{S}_{(c)}=S(\tilde{f}_1,...,\tilde{f}_C)_{(c)}$, $\tilde{S}_{(jc)}=\tilde{S}_{(c)}\cdot\frac{exp(\tilde{f}_j)}{\sum_{i=1}^C exp(\tilde{f}_i)}$, $\Sigma_{\tilde{f}\tilde{f}_j^{\partial_k}}$ denotes the transposed vector of covariances betweeen $\tilde{f}_j^{\partial_k}$ and the elements of $\tilde{f}$ and $\Sigma_{\tilde{f}}$ denotes the covariance matrix amongst the elements of $\tilde{f}$.
\end{corollary}

Now, treating the non-random elements in \eqref{expsimple} and \eqref{carymean} as constants, we can treat the respective right-hand sides as functions of $\tilde{f}$ and perform a second-order Taylor approximation around the mean. For binary classification, we obtain the following result:
\begin{theorem}
    The second-order Taylor approximation of \eqref{meanbinary} is:
    \begin{equation}\label{taylored}
        \begin{gathered}
             \mathbb{E}\left[\sigma'(\tilde{f})\cdot \tilde{f}^{\partial_k}\right]
             \\\approx\sigma'(\tilde{m})\tilde{m}^{\partial_k}+\frac{\tilde{k}}{2}\sigma'''(\tilde{m})\tilde{m}^{\partial_k}+\tilde{k}^{\partial_k}\sigma''(\tilde{m})  
        \end{gathered}
    \end{equation}
\end{theorem}
Notice that the $n$-th derivative of the sigmoid function evaluated at $x$, $\sigma^{(n)}(x)$, can be calculated recursively via

\begin{equation}
    \begin{gathered}
            \sigma^{(n)}(x)=\sum_{k=1}^{n+1}(-1)^{k+1}(k-1)!\\
            \cdot Stir(n+1,k)\sigma^(x)^k
    \end{gathered}
\end{equation}

where $Stir(\cdot,\cdot)$ denotes the Stirling Number of the Second Kind (\cite{minai1993derivatives}). 

For $C$-ary classification, the corresponding Taylor-series approximation is more complex but follows the same principles as the binary case. 

\begin{theorem}
    Denote by $\tilde{f}_j,\tilde{m}_j,\tilde{k}_j,\tilde{f}^{\partial_k}_j,\tilde{m}^{\partial_k}_j,\tilde{k}^{\partial_k}_j$ the marginal random variable and mean and kernel functions of the $j$-th SVGP (the $j$-th partial derivative SVGP) corresponding to an SVGP classifier as defined via \eqref{catlikelihood} and evaluated at an arbitrary $x$. Then, the second-order Taylor approximation of \eqref{meancary} is


\begin{equation}\label{multitaylor}
    \begin{gathered}
            \mathbb{E}\Bigg[S(\tf_1,...,\tf_C)_{(c)}\cdot \tf_c^{\partial_k}\\
            -S(\tf_1,...,\tf_C)_{(c)}
            \cdot \frac{\sum_{j=1}^C exp(\tf_j)\cdot \tf_j^{\partial_k}}{\sum_{j=1}^C exp(\tf_j)}\Bigg]\\
            \approx \kappa^k_{(c)}(\tilde{m}_1,...,\tilde{m}_C)+\frac{1}{2}\sum_{j=1}^C H^{\kappa^k}_{(c)}(\tilde{m}_1,...,\tilde{m}_C)_{(jj)}\cdot\tilde{k}_j.
    \end{gathered}
\end{equation}

\noindent where 

\begin{gather*}
\kappa^k_{(c)}(\tilde{f}_1,...,\tilde{f}_C) \\
= \tilde{S}_{(c)} \cdot \left\{\tilde{m}_c^{\partial_k}+\frac{\tilde{k}^{\partial_k}_c}{\tilde{k}_c} \left(\tilde{f}_c-\tilde{m}_c\right)\right\}\\
-\sum_{j=1}^C \tilde{S}_{(jc)}\left\{\tilde{m}_j^{\partial_k}+\frac{\tilde{k}^{\partial_k}_j}{\tilde{k}_j(} \left(\tilde{f}_j-\tilde{m}_j\right)\right\},
\end{gather*}

\noindent $\tilde{S}_{(c)}=S(\tilde{f}_1,...,\tilde{f}_C)_{(c)}$, $\tilde{S}_{(jc)}=\tilde{S}_{(c)}\cdot\frac{exp(\tilde{f}_j)}{\sum_{i=1}^C exp(\tilde{f}_i)}$ and $H^{\kappa^k}_{(c)}(\cdot,...,\cdot)_{(jj)}$ denotes $j$-th diagonal element of the Hessian of $\kappa^k_{(c)}(\cdot,...,\cdot)$.

\end{theorem}

As the Hessian of the target function is, presumably, hard to derive and handle in closed form, we will rely on Automatic Differentiation to evaluate it at the respective posterior means. Using the above approximation for the mean, we can easily approximate the mean of the integrated gradient by plugging in our estimates at the respective Riemann sum elements. 

For binary classification, we are therefore interested in each input's attribution 

\begin{equation}\label{binaryig}
    \begin{gathered}    
        \mathbb{E}[\hat{IG}(x)]=x_k\cdot\frac{1}{G}\sum_{g=1}^G\mathbb{E}\left[\frac{d \sigma(\tilde{f}(x))}{d x_k}\right]
    \end{gathered}
\end{equation}

where the respective $G$ means are approximated via \eqref{taylored}. In the multiclass case, we want to identify the attribution of each input towards the classifier's decision for the $c$-th class. Using the integrated gradient method for our multiclass GP setup, we are therefore interested in

\begin{equation}\label{naryig}
    \begin{gathered}    
        \mathbb{E}[\hat{IG}_c(x)]\\
        =x_k\cdot\frac{1}{G}\sum_{g=1}^G\mathbb{E}\left[\frac{\partial S(\tilde{f}_1(\frac{g}{G} x),...,\tilde{f}_C(\frac{g}{G} x))_{(c)}}{\partial x_k}\right].
    \end{gathered}
\end{equation}

The respective means in \eqref{naryig} are then approximated via \eqref{multitaylor}. Notice that it is also possible to estimate the necessary means in both \eqref{binaryig} and \eqref{naryig} via Monte-Carlo sampling \citep{kingma2013auto}. In the experiments section, we will consider both options and compare their results.

==> featatt/gpattribution_backup.tex <==
We now want to apply Integrated Gradient attribution to the case where $f$ is a single- or multi-output GP or, particularly for the non-Gaussian case, its element-wise transformation by an inverse-link function. Formally, we are create feature-wise attributions for

\begin{equation}\label{univariateoutput}
	g(f(\fatx)),\quad f(\fatx)\sim\mathcal{GP}(m(\fatx), k(\fatx,\fatx))
\end{equation}

to explain the output of a transformed single-output GP and

\begin{equation}\label{multioutput}
	\begin{gathered}
	G_c(F(\fatx)):=G(f^{(1)}(\fatx),...,f^{(C)}(\fatx)), \\
	f^{(j)}(\fatx)\sim\mathcal{GP}(m^{(j)}(\fatx), k^{(j)}(\fatx,\fatx))
	\end{gathered}
\end{equation}

to explain the c-th output of a transformed multi-output GP. In the case of classfication, where $g$ could be the probit or sigmoid and $G$ the softmax inverse link-function, the attributions from \eqref{univariateoutput} would then quantify the contribution of each feature towards the predicted class-probabilities. 

In the general case, analogously to Generalized Linear Models, $g(f(\fatx))$ can be used to model an arbitrary, meaningful summary statistic of the target likelihood, conditioned on $\fatx$ -  typically the conditional mean or the variance. Corresponding attributions then explain the contribution of each feature towards the model predicting the respective summary statistic.

In accordance with the single- and multi-output variants above, the corresponding Integrated Gradients are 

\begin{equation}\label{iggpuniv}
\begin{gathered}
\hat{IG}(\fatx,\fxb)_k^{g\circ f}= \frac{\fatx_k-\fxb_k}{R}\sum_{r=1}^T \frac{\partial g(f(\fxb+\frac{r}{R}\times(\fatx-\fxb)))}{\partial\fatx_k}\\
	=\frac{\fatx_k-\fxb_k}{R}\sum_{r=1}^B g'(f(\fatx_{(r)}))\cdot \frac{\partial}{\partial x_k} f(\fatx_{(r)})
\end{gathered}
\end{equation}

and

\begin{equation}\label{iggpmultiv}
\begin{gathered}
\hat{IG}(\fatx,\fxb)_k^{G_c\circ F}= \frac{\fatx_k-\fxb_k}{R}\sum_{r=1}^R \frac{\partial G_c(F(\fxb+\frac{r}{R}\times(\fatx-\fxb)))}{\partial\fatx_k}\\
=\frac{\fatx_k-\fxb_k}{R}\sum_{r=1}^R \nabla G_c(F(\fatx_{(r)}))^T\cdot \Jk F(\fatx_{(r)})
\end{gathered}
\end{equation}

where $\fatx_{(r)}:=\fxb+\frac{r}{R}\times(\fatx-\fxb)$ and $\Jk F$ denotes the $k$-th column of the Jacobian of $F$, i.e. the partial derivatives of each individual $f$ with respect to the $k$-th input feature. 

In order for the respective derivative processes to exist, we require the kernel functions $k(\cdot,\cdot)$ and $k^{(j)}(\cdot,\cdot),\quad j\in\{1,...,C\}$ to be twice differentiable with respect to both arguments. This condition can easily be verified for the Square-Exponential Kernel but also many other popular kernel functions and combinations thereof. See \cite{adler2010geometry}, p. 31, for reference.

With $f$ and $F$ being GPs, plugging $g(f)$ and $G(F)$ into \eqref{iggpuniv} and \eqref{iggpmultiv} essentially turns the Integrated Gradient into a stochastic process\footnote{Existence of such a process can easily be checked by observing that the operations involved preserve the Kolmogorov consistency properties of the underlying GPs}. The ideal outcome from here would be a complete description of the corresponding posterior processes

\begin{equation}\label{posterioriggp}
p\left(\hat{IG}(\cdot,\cdot')_k^{g\circ f}\bigg|y_1,...,y_N\right) \quad \text{and} \quad p\left(\hat{IG}(\cdot,\cdot)_k^{G_c\circ F}\bigg| \faty_1,...,\faty_N\right).
\end{equation}

In the trivial case of modelling the conditional mean of a Gaussian likelihood, where $g(\cdot)$ or $G(\cdot)$ are identity functions, \eqref{posterioriggp} is simply another GP whose mean and kernel functions are quickly obtained by summing the mean and kernel functions of the corresponding Riemann sum evaluations. Given the non-linear inverse link-functions involved in the general case, however, we simplify the problem by turning our attention to the generation of attributions for variational posterior evaluations at a given input. 

Hence, we are interested in the evaluation of the \textbf{deterministic} Integrated Gradient functions, given the respective SVGPs evalutated at the Riemann sum elements $\fatx_{(r)}=\fxb+r/R (\fatx - \fxb)$: 
\begin{equation}\label{iggpunivariational}
	q\left(IG(\fatx,\fxb)_k^{(g\circ f)}\right)=\int \delta\left(IG(\fatx,\fxb)_k^{(g\circ f)}\right)\cdot q\left(f(\fatx_{(1...R)}),f^{\partial_k}(\fatx_{(1...R)})\right)df(\fatx_{(1...R)}) df^{\partial_k}(\fatx_{(1...R)})
\end{equation}

and

\begin{equation}\label{iggpmultivariational}
	q\left(IG(\fatx,\fxb)_k^{(G_c\circ F)}\right)=\int \delta\left(IG(\fatx,\fxb)_k^{(G_c\circ F)}\right)\cdot q\left(F(\fatx_{(1...R)}),F^{\Jk}(\fatx_{(1...R)})\right)dF(\fatx_{(1...R)}) dF^{\Jk}(\fatx_{(1...R)}),
\end{equation}

where $\delta(\cdot)$ denotes the Dirac-delta function and we abused notation in \eqref{iggpmultivariational} by summarizing the individual $f^{(1)},...,f^{(C)}$ and their evaluations as $F$; $F^\Jk(\fatx_{(r)})$ denotes the collection of inidiviual partial derivative processes, $f^{(1)\partial_k}(\fatx_{(r)}),...,f^{(C)\partial_k}(\fatx_{(r)})$. Also, we summarized the random variables from individual GP evaluations $f(\fatx_{(1)}),f(\fatx_{(R)})$ as $f(\fatx_{(1...R)})$ and similarly for the random variables from the corresponding partial derivative GP evaluations.

Both \eqref{iggpuniv} and \eqref{iggpmultiv} are calculated as the sums of the random variables derived from the transformed GPs and their derivatives, times a factor $\frac{\fatx_k-\fxb_k}{R}$. We therefore shift our focus to the distribution of these individual summands,

\begin{equation}\label{iggpunivsummand}
	\begin{split}
		q\left(g'(f(\fatx_{(r)}))\cdot \frac{\partial}{\partial x_k} f(\fatx_{(r)})\right)&=\int \delta\left(g'(f(\fatx_{(r)}))\cdot \frac{\partial}{\partial x_k} f(\fatx_{(r)})\right)\cdot q\left(f(\fatx_{(r)})\right)df(\fatx_{(r)}) \\
		&=\int \delta\left(g'(f(\fatx_{(r)}))\cdot  f^{\partial_k}(\fatx_{(r)})\right)\cdot q\left(f(\fatx_{(r)},f^{\partial_k}(\fatx_{(r)}))\right)df(\fatx_{(r)})df^{\partial_k}(\fatx_{(r)})
	\end{split}
\end{equation}

and

\begin{equation}\label{iggpmultisummand}
\begin{split}
	q\left(\nabla G_c(F(\fatx_{(r)}))^T\cdot \nabla F(\fatx_{(r)})\right)&=\int \delta\left(\nabla G_c(F(\fatx_{(r)}))^T\cdot \Jk F(\fatx_{(r)}))\right)\cdot q\left(F(\fatx_{(r)})\right)dF(\fatx_{(r)}) \\
	&=\int \delta\left(\nabla G_c(F(\fatx_{(r)}))^T\cdot F^{\Jk}(\fatx_{(r)}))\right)\\
	&\quad\quad\quad\quad\cdot q\left(F(\fatx_{(r)}),F^{\Jk}(\fatx_{(r)})\right)dF(\fatx_{(r)})dF^\Jk(\fatx_{(r)}).
\end{split}
\end{equation}

In the case that $g(\cdot)$ or $G(\cdot)$ are identity functions as in standard GP regression with Gaussian likelihood, \eqref{iggpunivsummand} and \eqref{iggpmultisummand} clearly reduce to the corresponding GP partial derivative processes and, keeping the baseline $\fxb$ fixed,

\begin{equation}\label{iggausssingle}
	\hat{IG}(\cdot,\fxb)_k^{g\circ f} \sim \mathcal{GP}\left(m^{\hat{IG}_k^{g\circ f}}_{|\fxb}(\cdot),k^{\hat{IG}_k^{g\circ f}}_{|\fxb}(\cdot,\cdot)\right).
\end{equation}

with

\begin{equation}
	m^{\hat{IG}_k^{g\circ f}}_{|\fxb}(\fatx)=\frac{\fatx_k-\fxb_k}{R}\sum_{r=1}^R m_{|\fatf_U}^{\partial_k}\left(\fatx_{(r)}\right) 
\end{equation}

and

\begin{equation}
	k^{\hat{IG}_k^{g\circ f}}_{|\fxb}(\fatx,\fatx')=\left(\frac{\fatx_k-\fxb_k}{R}\right)\sum_{r,r'=1}^R k_{|\fatf_U}^{\partial_k}(\fatx_{(r)},\fatx_{(r')}')\left(\frac{\fatx_k'-\fxb_k}{R}\right).
\end{equation}

This follows directly from the fact linear transformations of multivariate Gaussian random variables are Gaussian themselves and the observation that the Integrated Gradient is a linear operation itself. The result for the multi-output case is analoguous to \eqref{iggausssingle}. 

The case for general $g(\cdot)$ and different likelihoods is far less convenient. Even in the single-output case we are already dealing with a linear-transform of products of marginals from a $2\times T$-dimensional multivariate distribution, where one factor of the product is non-linearly transformed by $g(\cdot)$, too. We can therefore safely assume that it is impossible to derive a closed form distribution for these finite-dimensional marginals, let alone the corresponding stochastic processes, implied by those marginals.

Since the (approximated) posterior mean is the typical point predictor in SVGP models, we consequently put our focus on generating attributions for 

\begin{equation}\label{meanssvgp}
	\meanofwrt{g(f(\fatx))}{q(f(\fatx))} \quad \text{and} \quad  \meanofwrt{G_c(F(\fatx))}{q(F(\fatx))}.
\end{equation}

By pulling the respective partial derivative operators into the mean, it is trivial to show that the mean of the Integrated Gradient processes and the Integrated Gradients for \eqref{meanssvgp} coincide:

\begin{equation}\label{meanofiguniv}
	\meanofwrt{\hat{IG}(\fatx,\fxb)_k^{g\circ f}}{q(f(\fatx_{(1...R)}),f^{\partial_k}(\fatx_{(1...R)}))} = \frac{\fatx_k-\fxb_k}{R}\sum_{r=1}^R \meanofwrt{g'(f(\fatx_{(r)}))\cdot f^{\partial_k}(\fatx_{(r)})}{q(f(\fatx_{(r)}),f^{\partial_k}(\fatx_{(r)}))}
\end{equation}

For the multi-output case, we proceed similarly and explicitly decompose the gradient dot-product into a sum of partial derivatives:

\begin{equation}\label{meanofigmulti}
	\begin{gathered}
		\meanofwrt{\hat{IG}(\fatx,\fxb)_k^{G_c\circ F}}{q(\fatF(\fatx_{(1...R)}),\fatF^{\Jk}(\fatx_{(1...R)}))} = \frac{\fatx_k-\fxb_k}{R}\sum_{r=1}^R \meanofwrt{\nabla G_c(F(\fatx_{(r)}))^T\cdot F^{\Jk}(\fatx_{(r)})}{q(\fatF(\fatx_{(r)}),\fatF^{\Jk}(\fatx_{(r)}))}\\
		=\frac{\fatx_k-\fxb_k}{R}\sum_{r=1}^R \sum_{j=1}^C\meanofwrt{\frac{\partial}{\partial f^{(j)}}G_c(f^{(1)}(\fatx_{(r)}),...,f^{(j)}(\fatx_{(r)})) f^{(r)\partial_k}(\fatx_{(r)})}{q(\fatF(\fatx_{(r)}),\fatF^{\Jk}(\fatx_{(r)}))}
	\end{gathered}
\end{equation}

Applying the fundamental theorem for line integrals to the above, similarly to the deterministic case, we get

\begin{equation}\label{lineintegraldiff}
	\begin{aligned}
		\sum_{k=1}^{M}\meanofwrt{\hat{IG}(\fatx,\fxb)_k^{g\circ f}}{q(f(\fatx_{(1...R)},f^{\partial_k}(\fatx_{(1...R)})))}&=\meanofwrt{\sum_{k=1}^{M}\hat{IG}(\fatx,\fxb)_k^{g\circ f}}{q(f(\fatx_{(1...R)}),f^{\partial_k}(\fatx_{(1...R)}))}\\
		&\approx\meanofwrt{g(f(\fatx))-g(f(\fxb))}{q(f(\fatx),f(\fxb))}\\
		&=\meanofwrt{g(f(\fatx))}{q(f(\fatx))}-\meanofwrt{g(f(\fxb))}{q(f(\fxb))}
	\end{aligned}
\end{equation}

as $R\rightarrow\infty$ and, therefore, $\hat{IG}(\fatx,\fxb)^{g\circ f}\rightarrow IG(\fatx,\fxb)^{g\circ f}$. The same conclusion can be drawn for the multi-output case. Later on, we will use these results to verify the correctness of the exact Integrated Gradient mean and empirically analyze the error for approximated Integrated Gradient means.

We will now state the main result of this paper, given additional simplifying notation as follows: 

$\mrfatfU$ and $\mrpkpfatfU$ denote the evaluation of the variational mean and partial derivative (with respect to the $k$-th input) mean functions at $\fatx_{(r)}$. $\krfatfU$ and $\krpkpfatfU$ denote corresponding evaluation of the variational kernel and partial derivative kernels at $\fatx_{(r)}$. $\krppkpfatfU$ denotes evaluation of the variational cross-covariance derivative kernel at $\fatx_{(r)}$.

The following Lemma is key to the remaining results and can trivially be proven with the law of total expectation\footnote{Write $\meanof{h(\fatx)y}=\meanof{h(\fatx)\meanof{y|\fatx}}$ and put in the formula for the conditional Gaussian mean.}:

\begin{lemma}\label{proplawtotalexp}
	Let $\bar{\fatx}$ denote a $C+1$-dimensional Gaussian random vector. Fix $\fatx$ and $y$, where $y$ is an arbitrary element of $\bar{\fatx}$ and $\fatx$ denotes the remaining elements of $\bar{\fatx}$ without $y$. Denote by $\mu_{\fatx},\mu_y$ the mean vector and mean scalar of $\fatx$ and $y$, by $\Sigma_{\fatx}$ the covariance matrix of $\fatx$ and by $\Sigma_{y\fatx}$ the transposed vector of covariances between $y$ and each element of $\fatx$.

Then, for a function $h:\mathbb{R}^C\mapsto A\subseteq\mathbb{R}$, with $h$ continuous, it follows that

$$\mathbb{E}\left[h(\fatx)\cdot y\right]=\mathbb{E}\left[h(\fatx)\cdot\left(\mu_y+
\Sigma_{y\fatx}\Sigma_{\fatx}^{-1}(\fatx-\mu_\fatx)\right)\right].$$

\end{lemma}

Using Lemma \ref{proplawtotalexp}, it is also possible to efficiently approximate the single-output Integrated Gradient means for arbitrary, differentiable inverse link-functions via Gaussian Quadrature. For exact results and an approximation of the softmax case, the following Theorem can be invoked:

\begin{theorem}
	Let $q(f)$ or $q(f^{(1)},...,f^{(R)})$ be SVGP variational posterior distributions of a single or multi-output and $g(\cdot)$ or $G(\cdot)$ non-linear inverse link-functions whose first derivative exists and is well-defined; in particular, let $g(\cdot)$ be either the square function, the natural exponential function, the Probit function $\Phi(\cdot)$ or the sigmoid function $s(cdot)$ and let $G(\cdot)$ be the softmax function. The corresponding mean Integrated Gradient attributions for a corresponding SVGP model as described above can then be calculated as follows: 

%\begin{table}[ht]
%	\small
%		\centering
    \begin{tabularx}{\textwidth}{l|X}
        \hline
		\small\textbf{Predictive mean} & \small\textbf{Integrated Gradient mean} $\meanof{\hat{IG}(\fatx,\fxb)_k^{g\circ f}}$ \\
        \hline
		\small $\meanofwrt{f(\fatx)^2}{q(f(\fatx))}$ & \small $=\frac{\fatx_k-\fxb_k}{R}\sum_{r=1}^R \left(2\mrfatfU\mrpkpfatfU+2\krpkpfatfU\right)$ \TBstrut \\
        \hline
		\small $\meanofwrt{\expof{f(\fatx)}}{q(f(\fatx))}$ &  \small $=\frac{\fatx_k-\fxb_k}{R}\sum_{r=1}^R\expof{\mrfatfU+0.5\krfatfU}\cdot\left(\mrpkpfatfU+\frackkppk\krfatfU\right)$  \TBstrut \\
        \hline
		\small $\meanofwrt{\Phi(f(\fatx))}{q(f(\fatx))} $ & \small $=\frac{\fatx_k-\fxb_k}{R}\sum_{r=1}^R\frac{1}{\sqrt{2\pi(1+\krfatfU)}}\gaussexp{\mrfatfU^2}{1+\krfatfU}\cdot\left(\mrpkpfatfU-\frackkppk\frac{\mrfatfU\krfatfU}{1+\krfatfU}\right)$ \TBstrut \\
		\hline
		\small $\meanofwrt{s(f(\fatx))}{q(f(\fatx)}$ & \small $\approx \frac{\fatx_k-\fxb_k}{R}\sum_{r=1}^R\left(s'(\mrfatfU)\mrpkpfatfU + \frac{1}{2}s'''(\mrfatfU)\mrpkpfatfU + \frackkppk s''(\mrfatfU)\right)$
 \TBstrut \\
		\hline
		\small $\meanofwrt{S_c(F(\fatx))}{q(F(\fatx))}$ & \small$\approx\begin{gathered} \frac{(\fatx_k-\fxb_k)}{R}\sum_{r=1}^R \left(\vphantom{\sum_{j\in\{1,...,C\}\setminus c}}H^k_{c(r)}(\fatm_{(r)|\fatf_U})+0.5\diag(\fatK_{(r)|\fatf_U})^T\diag(\nabla^2 H^k_{c(r)}(\fatm_{(r)|\fatf_U}))\right. \\\quad\quad\left.- \sum_{j\in\{1,...,C\}\setminus c} H_{cj(r)}^k(\fatm_{(r)|\fatf_U})+0.5\diag(\fatK_{(r)|\fatf_U})^T\diag(\nabla^2 H_{cj(r)}^k(\fatm_{(r)|\fatf_U}))\right)\end{gathered}$ \TBstrut \\
        \hline
    \end{tabularx}
%    \caption{}
%    \label{tab:mean_igs}
%\end{table}

where, in the approximation for the Integrated Gradient of a softmax model, 

\begin{equation}
	\begin{split}
		H^k_{c(r)}(\fatz)=	&=\Si{c}(\fatz)m^{(j)\partial_k}_{(r)|\fatf_U} - \Si{c}(\fatz)^2m^{(j)\partial_k}_{(r)|\fatf_U} + \Si{c}(\fatz)\left(\fatk^{(j)\partial_k}_{(r)|\fatf_U}\right)^T\fatK_{(r)|\fatf_U}^{-1}\fatz \\
		&\quad\quad- \Si{c}(\fatz)^2\fatz - \Si{c}(\fatz)\left(\fatk^{(j)\partial_k}_{(r)|\fatf_U}\right)^T\fatK_{(r)|\fatf_U}^{-1}\fatm_{(r)|\fatf_U} + \Si{c}(\fatz)^2\fatm_{(r)|\fatf_U}
	\end{split}
\end{equation}

and

\begin{equation}
	\begin{split}
		H^k_{cj(r)}(\fatz) &= S_c(\fatz)S_j(\fatz)m^{(j)\partial_k}_{(r)|\fatf_U}+S_c(\fatz)S_j(\fatz)\left(\fatk^{(j)\partial_k}_{(r)|\fatf_U}\right)^T\fatK_{(r)|\fatf_U}^{-1}\fatz \\
		&\quad\quad-S_c(\fatz)S_j(\fatz)\left(\fatk^{(j)\partial_k}_{(r)|\fatf_U}\right)^T\fatK_{(r)|\fatf_U}^{-1}\fatm_{(r)|\fatf_U}.
	\end{split}
\end{equation}
\end{theorem}






==> featatt/gpderivatives.tex <==
The goal of this section can be summarized as follows: For binary classification and evaluation datapoint $x$, we want to perform inference on

\begin{equation}\label{bin_svgp_attr}
    x_k\cdot\frac{1}{G}\sum_{g=1}^G\frac{\partial \sigma(\tilde{f}(\frac{g}{G} x))}{\partial x_k}.
\end{equation}

Equation \eqref{bin_svgp_attr} can be interpreted as the (random variable) integrated gradient of the SVGP posterior class probability. For $C$-ary classification, we proceed similarly:

\begin{equation}\label{cary_svgp_attr}
    x_k\cdot\frac{1}{G}\sum_{g=1}^G\frac{\partial S(\tilde{f}_1(\frac{g}{G} x),...,\tilde{f}_C(\frac{g}{G} x))_{(c)}}{\partial x_k}.
\end{equation}

Notice that, here, we are interested in the $k$-th integrated gradient with respect to the $c$-th class probability. Let us, for now, focus on a single summand of the integrated gradient and ignore the $\frac{g}{G}$ fraction. Applying the chain-rule on \eqref{bin_svgp_attr} and \eqref{cary_svgp_attr} then yields the following results:

\begin{equation}\label{explainbinary}
    \frac{\partial}{\partial x_k}\sigma(\tilde{f}(x))=\sigma'(\tilde{f}(x))\cdot \tilde{f}^{\partial_k}(x).
\end{equation}

\noindent for the binary case and 

\begin{equation}\label{explaincary}
    \begin{gathered}
    \frac{\partial}{\partial x_k}S(\tilde{f}_1(x),...,\tilde{f}_C(x))_{(c)}\\
    =S(\tilde{f}_1(x),...,\tilde{f}_C(x))_{(c)}\cdot \tilde{f}_c^{\partial_k}(x)-S(\tilde{f}_1(x),...,\tilde{f}_C(x))_{(c)}\\
    \cdot \frac{\sum_{j=1}^C exp(\tilde{f}_j(x))\cdot \tilde{f}_j^{\partial_k}(x)}{\sum_{j=1}^C exp(\tilde{f}_j(x))}
    \end{gathered}
\end{equation}

\noindent for $C$-ary classification problems (see Appendix A for a derivation). Here, $f^{\partial_k}(x)$ denotes the partial derivative of $f$ with respect to $x_k$. Particularly regarding \eqref{explaincary}, we are unlikely to find an analytical solution for the corresponding random variable, let alone for the sum of $G$ such variables for the integrated gradient. As a feasible alternative, we restrict ourselves on finding (approximate) solutions for the means of \eqref{explainbinary} and \eqref{explaincary}:

\begin{equation}\label{meanbinary}
    \mathbb{E}\left[\sigma'(\tilde{f}(x))\cdot \tilde{f}^{\partial_k}(x)\right]
\end{equation}

and

\begin{equation}\label{meancary}
    \begin{gathered}
            \mathbb{E}\Bigg[S(\tf_1(x),...,\tf_C(x))_{(c)}\cdot \tf_c^{\partial_k}(x)\\
            -S(\tf_1(x),...,\tf_C(x))_{(c)}\\
            \cdot \frac{\sum_{j=1}^C exp(\tf_j(x))\cdot \tf_j^{\partial_k}(x)}{\sum_{j=1}^C exp(\tf_j(x))}\Bigg].
    \end{gathered}
\end{equation}

By the linearity of the empirical integrated gradient, this allows us to ultimately derive approximate mean integrated gradients for both binary and multi-class classification. Let us now briefly touch some fundamental properties of GP derivatives and establish our key notation for subsequent derivations.\\


First, it is a well-known fact \citep{rasmussen2003gaussian}, that partial derivatives of GPs with respect to their input yield another GP with the following mean and kernel functions:

\begin{equation}
    \mathbb{E}\left[ f^{\partial_k}(\cdot)\right]:=m^{\partial_k}(\cdot) = \frac{\partial}{\partial x_k} m(\cdot)
\end{equation}

\noindent Similarly, we derive the covariance kernel $k^{\partial_k\partial_k'}(\cdot,\cdot)$ corresponding to $f^{\partial_k}$ as

\begin{equation}
    \begin{gathered}
        Cov\left[\frac{\partial}{\partial x_k} f(x),\frac{\partial}{\partial x'_k} f(x')\right]:=k^{\partial_k\partial_k'}(x,x')\\
        = \frac{\partial}{\partial x_k}\frac{\partial}{\partial x'_k}k(x,x')
    \end{gathered}
\end{equation}

\noindent Finally, for the covariance between the base GP $f$ and its partial derivative process:

\begin{gather}\label{crosscov}
    \begin{gathered}
    Cov\left[\frac{\partial}{\partial x_k} f(x), f(x')\right] := k^{\partial_k}(x,x')\\
    =\frac{\partial}{\partial x_k}k(x,x')\left(\equiv Cov\left[f(x),\frac{\partial}{\partial x'_k}  f(x')\right]\right)\\ \text{   (via symmetry of kernel functions)}
    \end{gathered}
\end{gather}


\noindent We now add $\partial_k$ super-scripts to annotate mean vectors and kernel Gram-matrices corresponding to the evaluation of derivative GPs, i.e. $K^{\partial_k\partial_k'}_{NN}$ denotes the kernel Gram-matrix corresponding to $k^{\partial_k\partial_k'}(x_i,x_j)$ for $x_i,x_j$ arbitrary row-vectors of a corresponding input matrix $X_N$.

With that, we are now ready to state the following helpful result:

\begin{proposition}
    Let $f\sim\mathcal{GP}(m(\cdot), k(\cdot, \cdot))$ and $f^{\partial_k}$ its corresponding $k$-th partial-derivative process. Let, additionally, $q(f_*,f_*^{\partial_k})=\int p(f_*,f_*^{\partial_k}|f_M)q(f_M)du$ be the joint variational process of both processes and $q(f_M)=\mathcal{N}(f_M|a,S)$ the variational inducing variable corresponding to $f$ at inducing locations $Z_M$. It then follows that
    
    \begin{equation}\label{gradpost}
        \begin{gathered}
        q(f_*^{\partial_k})\\
        =\int\int p(f_*,f_*^{\partial_k}|f_M)q(f_M)df_M\,df_*\\
        =\mathcal{N}(f_N^{\partial_k}|K_{*M}^{\partial_k}K_{MM}^{-1}a,\\
        K_{**}-\tilde{\Lambda}_{*M}^{\partial_k}(K_{MM}-S)\tilde{\Lambda}_{M*}^{\partial'_k})
        \end{gathered}
    \end{equation}
    
    where $\tilde{\Lambda}_{*M}^{\partial_k}=K^{\partial_k}_{*M}\left(K_{MM} - S\right)^{-1}$, $\tilde{\Lambda}_{M*}^{\partial'_k}=\left(K_{MM}  -S\right)^{-1}K^{ \partial_k'}_{M*}$.\newline
\end{proposition}

This follows from a trivial adjustment of the standard SVGP derivation by plugging in the respective derivative kernel matrices. The exact proof can be found in Appendix A. Another simple, albeit important result is the following:

\begin{proposition}\label{proplawtotalexp}
Let $\bar{X}$ denote a $C+1$-dimensional Gaussian random vector. Fix $X$ and $Y$, where $Y$ is an arbitrary element of $\bar{X}$ and $X$ denotes the remaining elements of $\bar{X}$ without $Y$. Denote by $\mu_X,\mu_Y$ the mean vector and mean scalar of $X$ and $Y$, by $\Sigma_{X}$ the covariance matrix of $X$ and by $\Sigma_{YX}$ the transposed vector of covariances between $Y$ and each element of $X$.

Then, for a function $g:\mathbb{R}^C\mapsto A\subseteq\mathbb{R}$, with $g$ continuous and $A$ bounded, it follows that

$$\mathbb{E}\left[g(X)\cdot Y\right]=\mathbb{E}\left[g(X)\cdot\left(\mu_Y+
\Sigma_{YX}\Sigma_{X}^{-1}(X-\mu_X)\right)\right].$$

\end{proposition}

\noindent This is a direct consequence of the law of total expectation

\begin{equation}\label{lawtotalexp}
    \mathbb{E}\left[g(X)\cdot 
    Y\right]=\mathbb{E}\left[\mathbb{E}[\left(g(X)\cdot Y)\right|X]\right]=\mathbb{E}\left[g(X)\cdot\mathbb{E}[Y|X]\right].
\end{equation}







==> featatt/gradientexplanations.tex <==
This sections introduces those concepts from explainable machine learning that are relevant to this paper. While the explainability has become a considerably popular research topic, standard, widely accepted definitions are still lacking. Hence, we will rely on the following definitions, based on \cite{understandingdeepnets}, for the remainder of this paper:

\begin{definition}\label{explanability}
    An \textbf{interpretation} is the mapping of an abstract concept into a domain that the human can make sense of. An \textbf{explanation} is the collection of features of the interpretable domain, that have contributed for a given example to produce a decision \textit{and a quantification of their influence}.
\end{definition}

Under this extended definition, a linear model is a suitable explanatory model:

\begin{equation}\label{linear}
    y = \beta_0 + \sum_{k=1}^K \beta_k x_k
\end{equation}

Here, the $x_k$ denote the 'features' as per our definition. Features could be, for example, pixels in an image, words in a sentence or a single row of feature columns in a tabular problem. The product $\beta_k x_k$ then expresses the quantification of their influence. We call $\beta_k x_k$ the \textbf{attribution} of the $k$-th feature at $x$.

For an arbitrary, $C^1$ differentiable function $f(\cdot)$, we can justify locally linear explanations and contributions via a first-order Taylor series expansion of $f(x)$ at $x_0$ , see for example \cite{deepinside}:

\begin{equation}\label{taylorexp}
    \begin{gathered}
            f(x)\approx f(x_0) + \left[\nabla f(x_0)\right]^T\cdot(x-x_0)\\
            = C + \left[\nabla f(x_0)\right]^T \cdot x = C + \sum_{k=1}^K \frac{\partial f(x_0)}{\partial x_{k}}\cdot x_k\\
            = \tilde{\beta}_0 + \sum_{k=1}^K \tilde{\beta}_k x_k
    \end{gathered}
\end{equation}

where $x_{0;k}$ denotes the $k$-th feature of $x_0$. Typically, we set $\frac{\partial f}{\partial x_{0;k}}=\frac{\partial f}{\partial x_{k}}$; the product $\frac{\partial f}{\partial x_{k}}\cdot x_k$ then takes the role of the \textit{attribution of the k-th feature}. We now write $f(\cdot)$ to explicitly denote functions and GPs with arbitrary input. For multivariate $f(\cdot)$ with $C$ outputs, we define, accordingly, the \textit{attribution of the k-th feature to the $c$-th output} as $\frac{\partial f_{(c)}}{\partial x_{k}}\cdot x_k$. Notice that we can equivalently treat $f_{(c)}(\cdot)$ as a univariate function.\\

As long as the respective features are within an interpretable domain as per Definition 1, \eqref{taylorexp} provides an explanation of the underlying model. Since we are only interested in the influence of each feature and not in an actual approximation of $f(x)$ via \eqref{taylorexp}, we can ignore $\tilde{\beta}_0$ for model explanation. While gradient-based explanations are only one possible option, the popularity of differentiable models and, mostly, cheap evaluations of gradients via automatic differentiation make them a highly suitable approach for modern machine learning.

An important contribution to gradient-based explanations has been made by \cite{axiomaticintegratedgradients}. The authors argue that the plain application of \eqref{taylorexp} for explaining complex, differentiable models can lead to logical inconsistencies, when considering a baseline input. To solve these issues, the authors propose \emph{integrated gradients} as an alternative that fulfills both of the above requirements. An \textit{empirical} integrated gradient is defined by a Riemann sum as follows:

\begin{equation}\label{igempirical}
    \hat{IG}_k(x) = (x_k-\tilde{x}_k)\frac{1}{G}\sum_{g=1}^{G}\frac{\partial f(\tilde{x}+\frac{g}{G}(x-\tilde{x}))}{\partial x_k}
\end{equation}

where $G$ denotes the number of partitions in the Riemann sum and $\tilde{x}=0$ is commonly chosen. We will adopt this setup for the remainder of this paper.

Notice that \eqref{igempirical} is linear in the model function we want to explain. This is particularly convenient for GP models, since GPs  are known to be closed under linear operations.


==> gaussprocs/dgps.tex <==
DGPs where first introduced in \cite{damianou2013deep} and apply the idea of stacking function approximators as in Deep Learning to GPs. Formally, let $f_1,...f_L$ be GP-distributed. A DGP is the functional composition of the $f_1,...f_L$, i.e. 


\begin{gather}
        F=f_L\circ\cdots \circ f_1 \sim\mathcal{DGP}\\
        f_l\sim\mathcal{GP}(m_l(\cdot),k_l(\cdot,\cdot))
\end{gather}
    


where the DGP depends on the mean and kernel functions of its component GPs. Similar to Neural Networks, it is possible and common to stack multiple GPs per DGP 'layer'. For simplicity, we won't cover this case. Still, all methods that we will introduce later on can naturally be extended to DGP layers with stacked GPs.

On the one hand, DGPs are considerably more flexible than plain GPs. This comes, however, at the cost of tractability of the probability distributions in play. This is particularly the case for the marginal likelihood

\begin{equation}\label{dgplikelihood}
    p(y|X)=\int_{f_1\times\cdots\times f_L}p(y|f_L)p(f_L|f_{L-1})\cdots p(f_1|X)df_1\cdots df_L
\end{equation}

which would be required for standard GP optimization. The same problem arises for the posterior predictive distribution which is, obviously, intractable as well. 

A convenient way to solve this issue is the introduction of inducing variables at each layer. In fact, this solution applies the same ideas as SVGPs and has been proven considerably successful for DGPs. We resort to the doubly variational approach demonstrated in \cite{salimbeni2017doubly} who construct a per-layer variational distribution as follows: 

\begin{equation}\label{dgpvar}
    q(f_l, u_l)=p(f_l|u_l;f_{l-1},Z_{l-1})q(u_l)
\end{equation}

where $Z_{l-1}$ denotes the inducing locations in analogy to SVGPs. We continue this parallelism and let $q(u_l)=\mathcal{N}(u_l|a_l,S_l)$ and have

\begin{gather}
    q(f_l)=\int_{u_l} q(f_l,u_l)du_l = \mathcal{N}(f_l|\Lambda_l a_l, K_{NN;l}-\Lambda_l(K_{MM;l}-S_l)\Lambda_l^T)\\
    
    \tilde{\Lambda}=K_{*N}(K_{NN}+I\sigma^2)^{-1}
    
\end{gather}

==> other_exports/riemann_approx_table.tex <==
\begin{tabular}{lllll}
\toprule
 & 50 & 500 & 1000 & 5000 \\
\midrule
Square & 0.0014 & 0.0001 & 0.0001 & 0.0000 \\
Exponential & 0.0078 & 0.0009 & 0.0004 & 0.0001 \\
Probit & 0.0008 & 0.0001 & 0.0001 & 0.0000 \\
Sigmoid (Gauss-Hermite) & 0.0006 & 0.0001 & 0.0000 & 0.0000 \\
Sigmoid (Taylor) & 0.0007 & 0.0004 & 0.0004 & 0.0004 \\
Softmax (Taylor) & 0.0013 & 0.0003 & 0.0002 & 0.0002 \\
\bottomrule
\end{tabular}

